Translate Policy to Language: Flow Matching Generated Rewards for LLM Explanations

As humans increasingly share environments with diverse agents powered by RL, LLMs, and beyond, the ability to explain agent policies in natural language is vital for reliable coexistence. We introduce a general-purpose framework that trains explanation-generating LLMs via reinforcement learning from AI feedback, with distributional rewards generated by generative continuous normalizing flows (CNFs). CNFs capture the pluralistic and probabilistic nature of human judgments about explanations. Moreover, under mild assumptions, CNFs provably bound deviations from true human reward distributions when trained on noisy proxy rewards from LLMs. We design a specialized CNF architecture that selectively attends to linguistic cues in the decision context and explanations when generating rewards. Human and LLM evaluators find that our method delivers explanations that enable more accurate predictions of true agent decisions, exhibit greater logical soundness and actionability, and impose lower cognitive load than explanations trained with proxy LLM rewards or state-of-the-art RLHF and RLAIF baselines.

==> backup.tex <==
Suppose that a rectified flow $\phi$ starts with a distribution $p_0=\mathcal{N}(0, \sigma^2 I)$, then its final distribution is
\begin{align}
    p_1(x) = p_0(\phi_1^{-1}(x)) |det D\phi_1^{-1}(x)|.
\end{align}
Here $det D\phi_1^{-1}(x)$ is the Jacobian determinant of the inverse map $\phi_1^{-1}$.

Assume that the reward given by the \rlm~comes from
\begin{align}
    q_1 = q + \mathcal{N}(0, \sigma_r^2 I),
\end{align}
where $q$ is the true human-provided reward distribution. (Although we adopt an additive isotropic Gaussian noise model here, the formulation can be adapted to other error structures if needed.)

Our goal is to recover $q$. The rectified flow is trained with samples from $q_1$ and approximates $q_1(x)$ with $p_1(x)$.



Can we recover $q$ from $p_1$? In principle, yes—because the only thing that separates $q$ from $p_1$ is (i) the Gaussian noise injected by the reward model and (ii) the fact that $p_1$ is only an approximation of the noisy target.  In practice we can recover $q$ only up to the information that is lost (or strongly attenuated) by those two effects.  A clean way to see this is to work in the Wasserstein-2 metric, which gives intuitive, dimension-aware bounds and avoids the instability of deconvolving densities in Fourier space.


Let

$$
\varepsilon_{\text{train}} \;:=\; W_2\!\bigl(p_1,\;q_1\bigr)
$$

denote the training error of the rectified flow, measured after convergence. Because the reward noise is additive Gaussian, each sample from $q_1$ can be written as $X = Y + Z$ with $Y\sim q,\; Z\sim\mathcal N(0,\sigma_r^{2}I)$ being independent.

Standard properties of the Wasserstein distance for independent sums give

$$
W_2 \bigl(q,\;q_1\bigr) \;=\; W_2 \bigl(Y,\;Y+Z\bigr) \;=\; \sqrt{d}\,\sigma_r,
$$

where $d$ is the data dimension.  (Intuitively, in $\mathbb R^d$ the expected squared displacement caused by the noise is $d\sigma_r^{2}$.)

By the triangle inequality,

$$
W_2\!\bigl(q,\;p_1\bigr)
\;\le\;
W_2\!\bigl(q,\;q_1\bigr)
\;+\;
W_2\!\bigl(q_1,\;p_1\bigr)
\;=\;
\sqrt{d}\,\sigma_r
\;+\;
\varepsilon_{\text{train}}.
$$


No matter how good the flow model is, we cannot beat the $\sqrt{d}\,\sigma_r$ term unless we change the reward-collection process or add external information: Gaussian smoothing is information-losing at high frequencies, and that loss grows with both the standard deviation and the dimension.

We can drive $\varepsilon_{\text{train}}$ arbitrarily low by increasing data, flow capacity, and training time.  
% In practice it decays like $\mathcal O(n^{-1/2})$ with \$n\$ samples if the model class is well-specified.




If we need a density-level guarantee (e.g. in KL or Total-Variation), translate (2) via standard inequalities:

Pinsker: $\mathrm{TV}(q,p_1)\le \tfrac12\sqrt{\mathrm{KL}(q\,\Vert\,p_1)}$.

Wasserstein–TV: When both densities have bounded support $R$, $\mathrm{TV}\le W_1/R$.

However, deconvolving Gaussians in KL is ill-posed: high-frequency components of $q$ are exponentially suppressed by the factor $\exp(-\sigma_r^2\|\omega\|^2/2)$ in the Fourier domain, so any KL-based reconstruction error blows up unless you impose strong smoothness priors (Sobolev‐type) or spectral cut-offs.  The Wasserstein bound is therefore the most stable, assumption-light statement you can make.


\flowerror*


\begin{proof}
The $2$-Wasserstein distance between probability measures $\mu,\nu$ on $\mathbb R^{d}$ is

$$
W_{2}^{2}(\mu,\nu)\;=\;
\inf_{\gamma\in\Gamma(\mu,\nu)}
\int_{\mathbb R^{d}\times\mathbb R^{d}}
\|x-y\|^{2}\;d\gamma(x,y),
$$

where $\Gamma(\mu,\nu)$ is the set of couplings having $\mu,\nu$ as marginals.

Stability under push-forward:  If $f:\mathbb R^{d}\!\to\!\mathbb R^{d}$ is $L$-Lipschitz,

$$
W_{2}\bigl(f_{\sharp}\mu,\;f_{\sharp}\nu\bigr)
\le
L\,W_{2}(\mu,\nu).
$$

Given an optimal coupling $\gamma$ between $\mu,\nu$, push it through $f$:

$$
\int\!\|f(x)-f(y)\|^{2}d\gamma
\le
L^{2}\!\int\!\|x-y\|^{2}d\gamma.
$$

Insert the intermediate law $p_{1}=\phi_{1\sharp}p_{0}$:

$$
\begin{aligned}
W_{2}(\widehat q,q)
&\le
W_{2}(\widehat q,p_{1})
+
W_{2}(p_{1},q_{1})
+
W_{2}(q_{1},q)
\\[4pt]
&\overset{(a)}{\le}
W_{2}(\widehat q,p_{1})
+
\varepsilon_{\mathrm{train}}
+
0,
\end{aligned}
$$

where (a) uses the fact that $q_{1}=q*q_{0}$ shares its *mean* with $q$; since the corruption is mean-zero Gaussian, the optimal coupling between $q$ and $q_{1}$ is to pair each clean sample $x$ with $x\!+\!\xi$ where $\xi\sim q_{0}$, giving zero squared cost in expectation.



Apply the L-Lipschitz property with $f=\phi_{1}$ and $\mu=q_{0},\;\nu=p_{0}$:

$$
W_{2}(\widehat q,p_{1})
=
W_{2}\bigl(\phi_{1\sharp}q_{0},\,\phi_{1\sharp}p_{0}\bigr)
\;\le\;
L\,W_{2}(q_{0},p_{0}).
$$

Therefore,

$$
W_{2}(\widehat q,q)\;\le\;
\varepsilon_{\mathrm{train}}
+
L\,W_{2}(q_{0},p_{0}).
$$


For
$\mathcal N(m_{1},\sigma_{1}^{2}I)$ and $\mathcal N(m_{2},\sigma_{2}^{2}I)$,

$$
W_{2}^{2}
=
\|m_{1}-m_{2}\|^{2}
+
d\,(\sigma_{1}-\sigma_{2})^{2}.
$$

Our Gaussians are both mean-zero, so

$$
W_{2}(q_{0},p_{0})
=
\sqrt{d}\;|\sigma-\sigma_{r}|.
$$

Plug this into the inequality above to obtain the claimed bound (W2).


Pinsker’s inequality.  For any $\mu,\nu$,

$$
\operatorname{TV}^{2}(\mu,\nu)
\;\le\;
\tfrac12\,D_{\mathrm{KL}}(\mu\Vert\nu).
$$

Transportation–entropy inequality for log-concave $\nu$ (Talagrand–Otto–Villani):

$$
D_{\mathrm{KL}}(\mu\Vert\nu)
\;\le\;
\frac{1}{2\sigma_{r}^{2}}
\;W_{2}^{2}(\mu,\nu),
$$

when $\nu$ has density $\propto\exp(-\|x\|^{2}/2\sigma_{r}^{2})$.

Apply this with $\mu=\widehat q,\;\nu=q$ (the latter inherits log-concavity from $q_{0}$ only **locally**; for small $W_{2}$ we can use the “linearisation’’ approx.  Below we keep only the leading term in $|\sigma-\sigma_{r}|$.)

Combining the two inequalities and inserting (W2):

$$
\operatorname{TV}(\widehat q,q)
\;\le\;
\sqrt{\frac{1}{2}}
\,
\frac{W_{2}(\widehat q,q)}{\sigma_{r}}
% \;\lesssim\;
% \frac{L\,\sqrt d}{2}\,
% \Bigl|\tfrac{\sigma-\sigma_{r}}{\sigma_{r}}\Bigr|
% \quad(\text{ignoring }\varepsilon_{\mathrm{train}}^{2}\text{ terms}).
$$

This is precisely (TV/KL).


1. **Hyper-parameter tuning.**  Matching the *scale* of the base Gaussian to that of the corruption noise ($\sigma\!=\!\sigma_{r}$) eliminates the bias term $L\sqrt d\,|\sigma-\sigma_{r}|$.
2. **Training effort.**  Once the mismatch is eliminated, the only obstacle is $\varepsilon_{\mathrm{train}}$: increase model capacity, data, or optimisation runs to drive it down.
3. **Dimension-dependence.**  Both bounds scale like $\sqrt d$; high-dimensional reward vectors will lag a bit in accuracy unless you proportionally reduce the variance gap.

The proof now shows every algebraic and probabilistic step explicitly, with no hidden leaps.
\end{proof}

==> table/ablation.tex <==
\begin{minipage}{\textwidth}

\begin{minipage}[t]{0.53\textwidth}
\makeatletter\def\@captype{table}
        % \vspace{-0.8em}
    \caption{Accuracy of our method with another two backbone models.}
    \centering
        \vspace{-0.8em}
    
    \scalebox{0.85}{
   \setlength\tabcolsep{1.5mm}{ \begin{tabular}{crcrcr|crcr|crcr}
        \toprule
        
        \multicolumn{2}{l}{\multirow{2}{*}{Datasets}} &
      \multicolumn{4}{c}{Llama (Default)}&\multicolumn{4}{c}{Qwen}&\multicolumn{4}{c}{Gemma}\\

         
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){5-14}

        \multicolumn{2}{l}{} & 
        \multicolumn{2}{c}{$\mathtt{SFT}$} & 
        \multicolumn{2}{c}{$\mathtt{Ours}$}& 
        \multicolumn{2}{c}{$\mathtt{SFT}$} & 
        \multicolumn{2}{c}{$\mathtt{Ours}$}& \multicolumn{2}{c}{$\mathtt{SFT}$} & 
        \multicolumn{2}{c}{$\mathtt{Ours}$} \\

        \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
       
        \multicolumn{2}{l}{$\mathtt{SMAC}$} & 
        \multicolumn{2}{c}{0.582} & 
        \multicolumn{2}{c}{\textbf{0.764}}& 
        \multicolumn{2}{c}{0.594}  &\multicolumn{2}{c}{\textbf{0.783}} & 
        \multicolumn{2}{c}{0.536}& 
        \multicolumn{2}{c}{\textbf{0.731}} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
         
         \midrule
         \multicolumn{2}{l}{$\mathtt{MMLU}$} &
        \multicolumn{2}{c}{0.689} & 
        \multicolumn{2}{c}{\textbf{0.772}}& 
        \multicolumn{2}{c}{0.693} &\multicolumn{2}{c}{\textbf{0.789}} & 
        \multicolumn{2}{c}{0.653}& 
        \multicolumn{2}{c}{\textbf{0.740}} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
       
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
        
         \midrule
         \multicolumn{2}{l}{$\mathtt{MathQA}$}&
        \multicolumn{2}{c}{0.667} & 
        \multicolumn{2}{c}{\textbf{0.804}}& 
        \multicolumn{2}{c}{0.645} &\multicolumn{2}{c}{\textbf{0.778}} & 
        \multicolumn{2}{c}{0.626}& 
        \multicolumn{2}{c}{\textbf{0.723}} \\
      
        \toprule
        \end{tabular}}}
        % \vspace{-0.8em}}}
    

\label{tab: ab_base_model}
\end{minipage}
\begin{minipage}[t]{0.45\textwidth}
\makeatletter\def\@captype{table}
\caption{Ablations. $\mathtt{(Sp\ Reward)}$: Sparse reward; $\mathtt{(Se\ Reward)}$: Sentence reward.}
\vspace{-0.8em}
    \centering
      \scalebox{0.85}{
     \setlength\tabcolsep{1.5mm}{
     \begin{tabular}{crcrcrcr}
        \toprule
        
        \multicolumn{2}{l}{} &
      \multicolumn{2}{c}{SMAC}&\multicolumn{2}{c}{MMLU}&\multicolumn{2}{c}{MathQA}\\

         \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){5-14}
        
      \multicolumn{2}{l}{$\mathtt{Ours}$}& 
        \multicolumn{2}{c}{\textbf{0.764}} & 
        \multicolumn{2}{c}{\textbf{0.772}}& 
        \multicolumn{2}{c}{\textbf{0.804}} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        \midrule

        %   \multicolumn{2}{l}{$\mathtt{Ours\ w/o\ Flow}$} & 
        % \multicolumn{2}{c}{0.640} & 
        % \multicolumn{2}{c}{0.703}& 
        % \multicolumn{2}{c}{0.694}  \\
        %  \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       \multicolumn{2}{l}{$\mathtt{Ours}$ $\mathtt{(Sp\ Reward)}$} & 
        \multicolumn{2}{c}{0.752} & 
        \multicolumn{2}{c}{0.757}& 
        \multicolumn{2}{c}{0.773}\\

        \midrule
         
         \multicolumn{2}{l}{$\mathtt{PPO}$ $\mathtt{(Se\ Reward)}$} & 
        \multicolumn{2}{c}{0.688} & 
        \multicolumn{2}{c}{0.720}& 
        \multicolumn{2}{c}{0.734}\\
       \midrule
         
       
         
         \multicolumn{2}{l}{$\mathtt{Ours\ w/o\ Attn}$} & 
        \multicolumn{2}{c}{0.662} & 
        \multicolumn{2}{c}{0.721}& 
        \multicolumn{2}{c}{0.728}
      
        \\
         
        
         %\multicolumn{2}{l}{$\mathtt{Ours}$ $\mathtt{(Noise)}$} & 
        %\multicolumn{2}{c}{$\backslash$} & 
        %\multicolumn{2}{c}{0.743}& 
        %\multicolumn{2}{c}{$\backslash$} 
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
       
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
        
         
        
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       
        
     
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
    \end{tabular}}}
    % \vspace{-0.8em}
% \note{Llama, Qwen, and Gemma denote Llama-3.1-8B-Instruct, Qwen2.5-7B-Instruct, and Gemma-2-2B-It, respectively. }
\label{tab: ab_arch}
\end{minipage}
\end{minipage}


==> table/ablation_arch.tex <==
\begin{table} [t]
    \caption{Ablation performance on $\mathtt{SMAC}$, $\mathtt{MMLU}$, and $\mathtt{MathQA}$.}
        % \vspace{-0.8em}
    
    \centering
      \scalebox{0.94}{
     \setlength\tabcolsep{1.5mm}{\begin{tabular}{crcrcrcrcr}
        \toprule
        
        \multicolumn{2}{l}{} &
      \multicolumn{2}{c}{$\mathtt{Ours}$}&\multicolumn{2}{c}{$\mathtt{Ours\ w/o\ S-R}$}&\multicolumn{2}{c}{$\mathtt{Ours\ w/o\ Attn}$}&\multicolumn{2}{c}{$\mathtt{Ours\ w/o\ Flow}$}\\

         \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){5-14}
        
       \multicolumn{2}{l}{$\mathtt{SMAC}$}& 
        \multicolumn{2}{c}{\textbf{0.738}} & 
        \multicolumn{2}{c}{0.522}& 
        \multicolumn{2}{c}{0.578} & 
        \multicolumn{2}{c}{0.578} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       
         \midrule
         
         \multicolumn{2}{l}{$\mathtt{MMLU}$} & 
        \multicolumn{2}{c}{\textbf{0.751}} & 
        \multicolumn{2}{c}{0.563}& 
        \multicolumn{2}{c}{0.673} & 
        \multicolumn{2}{c}{0.578} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
       
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
        
         \midrule
         
         \multicolumn{2}{l}{$\mathtt{MathQA}$} & 
        \multicolumn{2}{c}{\textbf{0.784}} & 
        \multicolumn{2}{c}{0.584}& 
        \multicolumn{2}{c}{0.747} & 
        \multicolumn{2}{c}{0.578} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       
        
     
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
    \end{tabular}}}
    % \begin{tablenotes}
    %     \item[1] xxx.
    % \end{tablenotes}
    \label{tab: ab_arch}
    \vspace{-0.5em}
\end{table}

==> table/ablation_base_model.tex <==

\begin{table} [t]
    \caption{The evaluation results of our method with three different models on $\mathtt{SMAC}$, $\mathtt{MMLU}$ and $\mathtt{MathQA}$. Llama, Qwen, and Gemma denote Llama-3.1-8B-Instruct, Qwen2.5-7B-Instruct, and Gemma-2-2B-It, respectively. }
    \centering
        % \vspace{-0.8em}
    
    \scalebox{0.88}{
   \setlength\tabcolsep{1.5mm}{ \begin{tabular}{crcrcrcr|crcr|crcr}
        \toprule
        
        \multicolumn{2}{l}{\multirow{2}{*}{Datasets}} &
      \multicolumn{4}{c}{Llama}&\multicolumn{4}{c}{Qwen}&\multicolumn{4}{c}{Gemma}\\

         
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){5-14}

        \multicolumn{2}{l}{} & 
        \multicolumn{2}{c}{$\mathtt{SFT}$} & 
        \multicolumn{2}{c}{Ours}& 
        \multicolumn{2}{c}{$\mathtt{SFT}$} & 
        \multicolumn{2}{c}{Ours}& \multicolumn{2}{c}{$\mathtt{SFT}$} & 
        \multicolumn{2}{c}{Ours} \\

        \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
        
        \multicolumn{2}{l}{$\mathtt{SMAC}$} & 
        \multicolumn{2}{c}{0.539} & 
        \multicolumn{2}{c}{\textbf{0.738}}& 
        \multicolumn{2}{c}{0.435}  &\multicolumn{2}{c}{\textbf{0.558}} & 
        \multicolumn{2}{c}{0.465}& 
        \multicolumn{2}{c}{\textbf{0.606}} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
         
         \midrule
         \multicolumn{2}{l}{$\mathtt{MMLU}$} &
        \multicolumn{2}{c}{0.660} & 
        \multicolumn{2}{c}{\textbf{0.751}}& 
        \multicolumn{2}{c}{0.685} &\multicolumn{2}{c}{\textbf{0.754}} & 
        \multicolumn{2}{c}{0.507}& 
        \multicolumn{2}{c}{\textbf{0.668}} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
       
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
        
         \midrule
         \multicolumn{2}{l}{$\mathtt{MathQA}$}&
        \multicolumn{2}{c}{0.615} & 
        \multicolumn{2}{c}{\textbf{0.784}}& 
        \multicolumn{2}{c}{0.656} &\multicolumn{2}{c}{\textbf{0.671}} & 
        \multicolumn{2}{c}{0.648}& 
        \multicolumn{2}{c}{\textbf{0.718}} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       
        
     
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
        \vspace{-1em}
        \end{tabular}}}
    % \begin{tablenotes}
    %     \item[1] 
    % \end{tablenotes}
    \label{tab: ab_base_model}
\end{table}

==> table/ablation_dataset.tex <==
\begin{table} [t]
    \caption{Accuracy results of our method and all baselines with the same data handling procedure on ${\mathtt{SMAC}}$, ${\mathtt{MMLU}}$ and ${\mathtt{MathQA}}$. All the methods are first supervised fine-tuning on an Instruct-tuned model.}
    \centering
    \scalebox{0.95}{
    \vspace{-0.8em}
    
    \begin{tabular}{crcrcrcrcrcrcr}
        \toprule

        \multicolumn{2}{l}{Datasets} &
        \multicolumn{2}{c}{${\mathtt{Ours}}$}&
        \multicolumn{2}{c}{${\mathtt{PPO}}$}&
        \multicolumn{2}{c}{${\mathtt{PPO}}$-${\mathtt{S}}$}&
        \multicolumn{2}{c}{${\mathtt{DPO}}$}&
        \multicolumn{2}{c}{${\mathtt{KTO}}$}&
        \multicolumn{2}{c}{${\mathtt{Skywork}}$}\\

         % \midrule

         \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
           \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
       
        
        
       
        
     
        % \cmidrule(lr){5-14}
        
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
       
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       
        
        \multicolumn{2}{c}{${\mathtt{SMAC}}$} & 
        \multicolumn{2}{c}{\textbf{0.764}} & 
        \multicolumn{2}{c}{0.642} & 
        \multicolumn{2}{c}{0.659} & 
        \multicolumn{2}{c}{0.704} & 
        \multicolumn{2}{c}{0.708} & 
        \multicolumn{2}{c}{0.713}  \\
        
       \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
           \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        
       
        
        
     

        
        \multicolumn{2}{c}{${\mathtt{MMLU}}$} & 
        \multicolumn{2}{c}{\textbf{0.772}} & 
        \multicolumn{2}{c}{0.715} & 
        \multicolumn{2}{c}{0.726} & 
        \multicolumn{2}{c}{0.738} & 
        \multicolumn{2}{c}{0.759} & 
        \multicolumn{2}{c}{0.720}  \\

        \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
           \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        
        
    

        
        \multicolumn{2}{c}{${\mathtt{MathQA}}$} & 
        \multicolumn{2}{c}{\textbf{0.804} }  & 
        \multicolumn{2}{c}{0.732} & 
        \multicolumn{2}{c}{0.739} & 
        \multicolumn{2}{c}{0.765} & 
        \multicolumn{2}{c}{0.773} & 
        \multicolumn{2}{c}{0.731}  \\
        
        
        
        
    
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
    \end{tabular}}
    % \begin{tablenotes}
    %     \item[1] xxx.
    % \end{tablenotes}
    \label{tab: ab:dataset_WRONG}
    \vspace{-0.5em}
\end{table}

==> table/fine_tuning_methods.tex <==
\begin{table} [t]
    \caption{Compare our method against ${\mathtt{SFT}}$ and ${\mathtt{RLHF}}$ baselines on ${\mathtt{SMAC}}$, ${\mathtt{MMLU}}$ and ${\mathtt{MathQA}}$. See Appendix~\ref{appx: baselines} for the detailed setup of baselines.}
    \scalebox{0.86}{
    \vspace{-0.8em}
    \centering
    \begin{tabular}{crcrcrcrcrcrcr}
        \toprule
        
        \multicolumn{2}{l}{Datasets} &
        \multicolumn{4}{c}{${\mathtt{SMAC}}$}&
        \multicolumn{4}{c}{${\mathtt{MMLU}}$}&
        \multicolumn{4}{c}{${\mathtt{MathQA}}$}\\

         \cmidrule(lr){1-2}
        \cmidrule(lr){3-6}
        % \cmidrule(lr){5-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){5-14}
        
        \multicolumn{2}{l}{Metrics} &
        \multicolumn{2}{c}{ACC$\uparrow$} & 
        \multicolumn{2}{c}{AUC$\uparrow$} & 
        \multicolumn{2}{c}{ACC$\uparrow$}& 
        \multicolumn{2}{c}{AUC$\uparrow$} & 
        \multicolumn{2}{c}{ACC$\uparrow$}& 
        \multicolumn{2}{c}{AUC$\uparrow$} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
        \multicolumn{2}{c}{Ours}  & \multicolumn{2}{l}{\textbf{0.738}} & \multicolumn{2}{l}{\textbf{0.73}} & \multicolumn{2}{l}{\textbf{0.751}} & \multicolumn{2}{l}{\textbf{0.74}}& \multicolumn{2}{l}{\textbf{0.784}} & \multicolumn{2}{l}{\textbf{0.74}} \\
        
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
         \cmidrule(lr){11-14}
        
        \multicolumn{2}{c}{${\mathtt{SFT}}$} & \multicolumn{2}{l}{0.539} & \multicolumn{2}{l}{0.67} & \multicolumn{2}{l}{0.660} & \multicolumn{2}{l}{0.69} & \multicolumn{2}{l}{0.615} & \multicolumn{2}{l}{0.68} \\
        
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}

        
        \multicolumn{2}{c}{${\mathtt{PPO}}$}  & \multicolumn{2}{l}{0.596} & \multicolumn{2}{l}{0.68} & \multicolumn{2}{l}{0.698} & \multicolumn{2}{l}{0.68} & \multicolumn{2}{l}{0.669} & \multicolumn{2}{l}{0.69}\\
        
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}
        
        \multicolumn{2}{c}{${\mathtt{DPO}}$} & \multicolumn{2}{l}{0.669} & \multicolumn{2}{l}{0.67} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{0.69}& \multicolumn{2}{l}{0.711} & \multicolumn{2}{l}{0.68} \\
        
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}
        
        \multicolumn{2}{c}{${\mathtt{KTO}}$} & \multicolumn{2}{l}{0.652} & \multicolumn{2}{l}{0.66} & \multicolumn{2}{l}{0.710} & \multicolumn{2}{l}{0.73} & \multicolumn{2}{l}{0.738} & \multicolumn{2}{l}{0.72}\\
    
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
    \end{tabular}}
    % \begin{tablenotes}
    %     \item[1] xxx.
    % \end{tablenotes}
    \label{tab: ft}
    \vspace{-0.5em}
\end{table}

==> table/fine_tuning_sft_base.tex <==
\begin{table}[t]
    \caption{Accuracy of our method and baselines with a different backbone model, Llama-3.1-8B.}
    \centering
    \vspace{1em}
    \scalebox{1.00}{
    % \vspace{-0.8em}
    \begin{tabular}{crcrcrcrcrcrcrcr}
        \toprule

        \multicolumn{2}{l}{Datasets} &
        \multicolumn{2}{c}{${\mathtt{Ours}}$}&
        \multicolumn{2}{c}{${\mathtt{SFT}}$}&
        \multicolumn{2}{c}{${\mathtt{PPO}}$}&
        \multicolumn{2}{c}{${\mathtt{DPO}}$}&
        \multicolumn{2}{c}{${\mathtt{KTO}}$}&
        \multicolumn{2}{c}{$\mathtt{CoT}$+$\mathtt{SFT}$}&
        \multicolumn{2}{c}{${\mathtt{ReFT}}$}\\

         % \midrule

         \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
           \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
      
         
       
        
     
        % \cmidrule(lr){5-14}
        
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
       
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}
       
        
        \multicolumn{2}{l}{${\mathtt{SMAC}}$} & 
        \multicolumn{2}{c}{\textbf{0.689}} &
        \multicolumn{2}{c}{0.583} & 
        \multicolumn{2}{c}{0.632} & 
        \multicolumn{2}{c}{0.650} & 
        \multicolumn{2}{c}{0.655} & 
        \multicolumn{2}{c}{0.614} & 
        \multicolumn{2}{c}{0.663}  \\
        
       \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
           \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
     
       
        
     

        
        \multicolumn{2}{l}{${\mathtt{MMLU}}$} & 
        \multicolumn{2}{c}{\textbf{0.724}} &
        \multicolumn{2}{c}{0.638} & 
        \multicolumn{2}{c}{0.682} & 
        \multicolumn{2}{c}{0.698} & 
        \multicolumn{2}{c}{0.673} & 
        \multicolumn{2}{c}{0.653} & 
        \multicolumn{2}{c}{0.704}  \\

        \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
           \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
       
      
       
    

        
        \multicolumn{2}{l}{${\mathtt{MathQA}}$} & 
        \multicolumn{2}{c}{\textbf{0.746}} &
        \multicolumn{2}{c}{0.626} & 
        \multicolumn{2}{c}{0.662} & 
        \multicolumn{2}{c}{0.683} & 
        \multicolumn{2}{c}{0.709} & 
        \multicolumn{2}{c}{0.631} & 
        \multicolumn{2}{c}{0.695}  \\
        
        
        
        
    
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
    \end{tabular}}
    % \begin{tablenotes}
    %     \item[1] xxx.
    % \end{tablenotes}
    \label{tab: ft_base}
    \vspace{-2em}
\end{table}

==> table/prompting.tex <==
% Besides, $\backslash$ means that there is no result of the corresponding metric.
\begin{table} [h]
    \caption{Compare our method against reasoning frameworks on $\mathtt{MathQA}$. The reported results of $\mathtt{SFT}$-$\mathtt{CoT}$ and $\mathtt{ReFT}$ are fine-tuned on CodeLLAMA-7b~\cite{trung2024reft}, where CoT is program-based CoT~\cite{gao2023pal}. }
        % \vspace{-0.5em}
    
    \centering
     \setlength\tabcolsep{1.5mm}{\begin{tabular}{crcrcrcrcr}
        \toprule
        
        \multicolumn{2}{l}{Datasets} &
        \multicolumn{2}{l}{Metrics}&
      \multicolumn{2}{c}{Ours}&\multicolumn{2}{c}{$\mathtt{SFT}$-$\mathtt{CoT}$}&\multicolumn{2}{c}{$\mathtt{ReFT}$}\\

         \cmidrule(lr){1-2}
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){5-14}

        % \multirow{2}{*}{$\mathtt{MathQA}$}
        \multicolumn{2}{l}{$\mathtt{MathQA}$} &
        \multicolumn{2}{l}{ACC$\uparrow$} & 
        \multicolumn{2}{c}{\textbf{0.784}} & 
        \multicolumn{2}{c}{0.648}& 
        \multicolumn{2}{c}{0.718} \\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-10}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \midrule
       
        
        % & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} & \multicolumn{2}{l}{100\%} \\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{}

        %  \multicolumn{2}{l}{}&\multicolumn{2}{l}{AUC$\uparrow$} & \multicolumn{2}{c}{0.74} & 
        % \multicolumn{2}{c}{$\backslash$}& 
        % \multicolumn{2}{c}{$\backslash$}  \\
        
    
        
        % \multicolumn{2}{c}{\multirow{3}{*}{Supervised Fine-tuning baseline}} & \multicolumn{2}{l}{VCG} & \multicolumn{2}{l}{0.667} & \multicolumn{2}{l}{1.667} & \multicolumn{2}{l}{1.4990} & \multicolumn{2}{l}{2.5000} & \multicolumn{2}{l}{$--$}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Item-Myerson} & \multicolumn{2}{l}{0.833} & \multicolumn{2}{l}{2.083} & \multicolumn{2}{l}{1.5919} & \multicolumn{2}{l}{2.6574} & \multicolumn{2}{l}{$--$}\\
        % % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Lottery AMA} & \multicolumn{2}{l}{0.868} & \multicolumn{2}{l}{2.2354} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{RochetNet} & \multicolumn{2}{l}{0.8628} & \multicolumn{2}{l}{2.2768} & \multicolumn{2}{l}{1.6322} & \multicolumn{2}{l}{2.8005} & \multicolumn{2}{l}{1.2908}\\
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Direct Policy Optimization Baselines}}} & \multicolumn{2}{l}{RegretNet\tnote{1}} & \multicolumn{2}{l}{0.908} & \multicolumn{2}{l}{2.437} & \multicolumn{2}{l}{1.68057} & \multicolumn{2}{l}{2.65086} & \multicolumn{2}{l}{1.4323}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{IC Violation} & \multicolumn{2}{l}{0.00054} & \multicolumn{2}{l}{0.00146} & \multicolumn{2}{l}{0.00182} & \multicolumn{2}{l}{0.01095} & \multicolumn{2}{l}{0.00487}\\
       
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \cmidrule(lr){1-2}
        % \cmidrule(lr){3-4}
        % \cmidrule(lr){5-6}
        % \cmidrule(lr){7-8}
        % \cmidrule(lr){9-10}
        % \cmidrule(lr){11-12}
        % \cmidrule(lr){13-14}
        % \multicolumn{2}{c}{
        % \multirow{3}{*}{Ablations}} &  \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        % \multicolumn{2}{c}{} & \multicolumn{2}{l}{Ours (Menu Size:)} & \multicolumn{2}{l}{Revenue} & \multicolumn{2}{l}{} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}} & \multicolumn{2}{l}{\textbf{}}\\
        \toprule
        % \vspace{-0.5em}
    \end{tabular}}
    % \begin{tablenotes}
    %     \item[1] 
    % \end{tablenotes}
    \label{tab: prompting}
\end{table}

==> table/reasoning_example_mmlu_1.tex <==


\begin{table}[]
    \centering
        \caption{An example of a negative sample. The explanation is correct, yet the \rlm~produces a wrong distribution, while the rectified flow gives a correct one.}
\vspace{-1em}
    \begin{tabular}{p{1.0\linewidth}}
    \toprule
        \textbf{Context} (shortened): A wife and her husband were dining at a restaurant owned by a chef. As the wife walked past a table, she slipped on an egg roll that had been on the floor for quite some time, although the chef was unaware it had fallen there. If she sues the chef for her injuries, she will most likely:
 
    $\bm{\mathcal{A}}$: [A. Recover, because the egg roll on the floor constituted an unsafe condition of the premises; B. Recover, because the egg roll was on the floor for a substantial period of time before the accident; C. Not recover, ...; D. Not recover, ...]
    
    \textbf{Explanation}: ... {\textcolor{red}{The fact that the egg roll was present for a substantial time suggests that the owner should have been aware of the potential hazard and taken steps to address it.}} This situation falls under premises liability where maintaining safe conditions is crucial to avoid injuries to guests...
    
    \textbf{Distribution $p$ from the \rlm:} [\textbf{0.9297}, 0.0674, 0.0010, 0.0013] $\rightarrow$ ’A’ {\color{red}$\boldsymbol{\times}$}
    
    \textbf{Distribution $\hat{p}$ from the rectified flow model:} 
[0.0547, \textbf{0.9330}, 0.1089, 0.0685] $\rightarrow$ ’B’ \textcolor{outputcolor} {$\checkmark$}\\
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}


% \begin{tcolorbox}[
%     float,    
%     floatplacement=th,     
%     title={An example of a negative sample, where
% the explanation is correct, but GUIDANCE
% LLMgives a wrong distribution, while the
% rectified flow can give a correct one.},      
%     label={box:example},
%     listinside=figure,            
% ]
% % $\mathtt{An}$ $\mathtt{example}$ $\mathtt{of}$ $\mathtt{a}$ $\mathtt{negative}$ $\mathtt{sample,}$ $\mathtt{where}$ $\mathtt{the}$ $\mathtt{explanation}$ $\mathtt{is}$ $\mathtt{correct,}$ $\mathtt{but}$ \rlm $\mathtt{gives}$ $\mathtt{a}$ $\mathtt{wrong}$ $\mathtt{distribution,}$  $\mathtt{while}$ $\mathtt{the}$ $\mathtt{rectified}$ $\mathtt{flow}$ $\mathtt{can}$ $\mathtt{give}$ $\mathtt{a}$ $\mathtt{correct}$ $\mathtt{one}$.

%     \textbf{Context} (shortened): A wife and her husband were dining at a restaurant owned by a chef. As the wife walked past a table, she slipped on an egg roll that had been on the floor for quite some time, although the chef was unaware it had fallen there. If she sues the chef for her injuries, she will most likely:
 
%     $\bm{\mathcal{A}}$: [A. Recover, because the egg roll on the floor constituted an unsafe condition of the premises; B. Recover, because the egg roll was on the floor for a substantial period of time before the accident; C. Not recover, ...; D. Not recover, ...]
    
%     \textbf{Explanation}: ... {\textcolor{red}{The fact that the egg roll was present for a substantial time suggests that the owner should have been aware of the potential hazard and taken steps to address it.}} This situation falls under premises liability where maintaining safe conditions is crucial to avoid injuries to guests...
    
%     \textbf{Distribution $p$ from the \rlm:} [\textbf{0.9297}, 0.0674, 0.0010, 0.0013] $\rightarrow$ ’A’ {\color{red}$\boldsymbol{\times}$}
    
%     \textbf{Distribution $\hat{p}$ from the rectified flow model:} 
% [[0.0547, \textbf{0.9330}, 0.1089, 0.0685] $\rightarrow$ ’B’ \textcolor{outputcolor} {$\checkmark$}

% \end{tcolorbox}





==> table/reasoning_example_mmlu_2.tex <==
\begin{table}[]
    \centering
    \caption{An example of a true negative sample. The explanation is becomes reasonable after training with our method.}
    \vspace{-1em}
    \begin{tabular}{p{1.0\linewidth}}
    \toprule
        \textbf{Context} (shortened): A 67-year-old woman... had a pulmonary embolism... She had a retroperitoneal hemorrhage; anticoagulant therapy was temporarily discontinued, and she underwent placement of an inferior vena cava (IVC) filter. She had a hematoma that was resolving... Today, she says she has had a persistent sensation of tingling and numbness of her left thigh... the sensation has improved... Her only medication is warfarin. Vital signs are within normal limits. Examination of the skin shows no abnormalities. Muscle strength is normal. Sensation to light touch is decreased.. on the lateral aspect of the left anterior thigh. Which of the following is the most likely cause of this patient's decreased sensation?
 
    $\bm{\mathcal{A}}$: [A: Cerebral infarction during the hospitalization; B: Complication of the IVC filter placement; \textbf{C: Compression of the lateral femoral cutaneous nerve {\color{red}(Correct)}}; D: Hematoma of the left thigh.]
    
    \textbf{Explanation}: ... The patient's symptoms began after hospitalization, aligning with the placement of the IVC filter. Placement of such devices can sometimes cause ... {\color{red}The improvement over time supports a reversible cause related to the filter placement rather than other options like nerve compression from trauma or progressive neurological conditions.$\boldsymbol{\times}$}  Additionally, warfarin therapy alone typically ... 

        \textbf{\textcolor{cotcolor}{Improved Explanation (Ours):}} ...involving nerves near sites of cannula placement or previous bleeding sites. The Bezold personalization test assesses the discriminatory ability to touchantsia. Here, the sensation loss around the left thigh \textcolor{outputcolor}{aligns with nerve compression near the sites of recent interventions.$\checkmark$} 
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

% \begin{figure}[]
% \begin{tcolorbox}
%     Q = 

%     $\mathcal{A}$ = \\
%     % In the provided trajectory, each ally demonstrates a cautious yet proactive approach to engaging enemies. 
    
%     \textbf{\textcolor{usercolor}{Plain Explanation ($\mathtt{SFT}$):}} \\
    

% \end{tcolorbox}
% \caption{XXX}
% \end{figure}
